Cluster Specific Representation Learning

Representation learning aims to extract meaningful lower-dimensional embeddings from data, known as representations. Despite its widespread application, there is no established definition of a ``good'' representation. Typically, the representation quality is evaluated based on its performance in downstream tasks such as clustering, de-noising, etc. However, this task-specific approach has a limitation where a representation that performs well for one task may not necessarily be effective for another. This highlights the need for a more agnostic formulation, which is the focus of our work. We propose a downstream-agnostic formulation: when inherent clusters exist in the data, the representations should be specific to each cluster. Under this idea, we develop a meta-algorithm that jointly learns cluster-specific representations and cluster assignments. As our approach is easy to integrate with any representation learning framework, we demonstrate its effectiveness in various setups, including Autoencoders, Variational Autoencoders, Contrastive learning models, and Restricted Boltzmann Machines. We qualitatively compare our cluster-specific embeddings to standard embeddings and downstream tasks such as de-noising and clustering. While our method slightly increases runtime and parameters compared to the standard model, the experiments clearly show that it extracts the inherent cluster structures in the data, resulting in improved performance in relevant applications.

==> sections/method.tex <==
\section{Cluster Specific Models}

% \subsection{Cluster Specific (Variational-) Autoencoders}

We now formalize the general idea outlined in Figure~\ref{fig: TAE illustration}by explicitly stating the optimization problems we consider throughout this work. We outline for each optimization objective how it can be extended to a cluster specific version.

\subsection{Autoencoders}
    
    \textbf{Reconstruction based losses} build on the idea of mapping data into a lower dimensional latent space and then project it back into the initial dimensionality. The model is then optimized by minimizing the difference between he data and the reconstruction. Main considered examples we consider here are AEs and Variational Autoencoders. 
    One of the most common approaches in deep learning for obtaining latent representations are Autoencoders (AE) \cite{Kramer1991AIChE_AE} where the idea is to map the data into a lower dimensional space using an \emph{encoder} and then back into the original space using a \emph{decoder}. The encoder and encoder are optimized by minimizing the \emph{reconstruction error}.
 The empirical success of autoencoders has given rise to a large body of work, developed for task specific regularisation (e.g. \cite{yang2017towards}), as well as for a wide range of applications such as image denoising \cite{buades2005review}, clustering \cite{yang2017towards} or natural language processing \cite{zhang2022survey}.


The same idea is applied to the decoder such that the new overall model for the \emph{Partial Tensorized Autoencoder (PTAE)} is defined as
\begin{align}\label{eq:PTAE}
&\min_{\substack{\{\Phi_j, \Psi_j\}^k_{j},\\\Theta,\Omega,S}}
\sum^n_{i=1}  \sum^k_{j = 1}S_{j,i}\left[\norm{\tilde{X}_{i,j} - \hat{x}_{i,j}
}^2 
- \lambda p(X_i)
\right]\\
&\text{s.t. ~ } 1_k^TS = 1_n^T,\ S_{j,i} \geq 0,\nonumber\\
&\text{and ~ }\hat{x}_{i,j}:=f_{\Theta}(f_{\Phi_j}(g_{\Psi_j}(g_{\Omega}(\tilde{X}_{i,j})))).\nonumber
\end{align}
with $\tilde{X}_{i,j}:=X_i-C_j$ and 
where $S$ is a $k \times n$ matrix, such that $S_{j,i}$ is the probability that data point $i$ belongs to class $j$, $g_{\Psi_j}( \cdot )$ and $f_{\Phi_j}( \cdot )$ are the \emph{encoder }and the \emph{decoder} functions respectively specific to points in class $j$, and $C_j$ is a parameter centering the data passed to each autoencoder specific to class $j$.
Specifically a $k$-means \cite{Macqueen67somemethods} penalty is considered to enforce a cluster friendly structure in the latent space (similar to the one proposed in \cite{Bo2017k_means_friendly}).
 $\lambda$ determines the strength of the penalty, that is chosen depending on the task or desired properties of the parameters.
This general architecture allows specifically choose the trade-off between giving more importance to the shared or to the cluster specific part of the function. 
For the remainder of the paper we consider the setting where $g_{\Psi_j}$ only consists of one fully connected layer and the rest of the encoder is shared. This is the model with the smallest number of parameters while still preserving the overall idea of tensorization. The underlying idea is that even between data from different clusters the 


\subsection{Variational Autoencoders}

A Variational Autoencoder (VAE) is a generative model that employs neural networks to learn the underlying distribution of data. It combines the principles of variational inference and autoencoders. Formally, let $ {x} $ represent the observed data and $ {z_j} $ the latent variables. The VAE consists of two main components:
\emph{Encoder (Inference Model)}: $ q_{\Phi_j}({z_j}|{x}) $, a neural network parameterized by $ \Phi_j $, which approximates the posterior distribution of the latent variables given the observed data.
\emph{Decoder (Generative Model)}: $ p_{\Psi_j}({x}|{z_j}) $, a neural network parameterized by $ \Psi_j $, which models the likelihood of the observed data given the latent variables.

The VAE optimizes the Evidence Lower Bound (ELBO) on the marginal likelihood $ p_{\theta}({x}) $:
\begin{align*}
% \log p_{\Psi_j}({x}) \geq 
\mathbb{E}_{q_{\Phi_j}({z_j}|{x})}[\log p_{\Psi_j}({x}|{z})] - \text{KL}(q_{\Phi_j}({z_j}|{x}) \| p({z_j}))    
\end{align*}
where $ \text{KL} $ denotes the Kullback-Leibler divergence, and $ p({z_j}) $ is the prior distribution over the latent variables, typically a standard Gaussian $ \mathcal{N}({0}, {I}) $.

The first term is referred to the \emph{Reconstruction Term} and the second one as the \emph{Regularization Term}. In practice this optimization problem is implemented as follows:
\todo[inline]{add exact VAE formulation}
\todo[inline]{add discussion on center problem}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.24\linewidth]{figures/VAE/vae_lr0.001_ep200_reg0.5_mseFalse_loutFalse_clustidNone.pdf}
    \includegraphics[width=0.24\linewidth]{figures/VAE/tvae_lr0.001_ep500_reg0.1_mseFalse_loutFalse_clustid0.pdf}
    \includegraphics[width=0.24\linewidth]{figures/VAE/tvae_lr0.001_ep500_reg0.1_mseFalse_loutFalse_clustid1.pdf}
    \includegraphics[width=0.24\linewidth]{figures/VAE/tvae_lr0.001_ep500_reg0.1_mseFalse_loutFalse_clustid2.pdf}
    \caption{Sigmoid output, BCE loss, MNIST, FCN}
    \label{fig:vae_latent_space}
\end{figure*}

% The ELBO comprises two terms:

% 1. **Reconstruction Term**: $ \mathbb{E}_{q_{\phi}({z}|{x})}[\log p_{\theta}({x}|{z})] $, which encourages the model to reconstruct the observed data accurately.
% 2. **Regularization Term**: $ \text{KL}(q_{\phi}({z}|{x}) \| p({z})) $, which regularizes the encoder to keep the latent distribution close to the prior.

% The VAE is trained by maximizing the ELBO with respect to the parameters $ \phi $ and $ \theta $. This training procedure allows the model to generate new, similar data samples by sampling from the learned latent space distribution $ p({z}) $ and decoding through $ p_{\theta}({x}|{z}) $.

\subsection{ Self Supervised Learning}
  \textbf{Embedding based losses} build on the idea that certain properties between embeddings of different data points should be preserved. Most notably points that are similar\footnote{We later discuss in Section~\ref{} how exactly we define 'similar'.} in the features space should be close to each other in the latent space. This main idea is formalized through (non)-contrastive losses in Self supervised learning.
    This concept has been established in recent years as an important method between supervised and unsupervised learning as it does not require explicit labels but relies on implicit knowledge of what makes  samples semantically close to others. Therefore SSL builds on inputs and inter-sample relations $(X , \overline{X})$, where $\overline{X}$ is often constructed through data-augmentations of $X$ known to preserve input semantics such as additive noise or horizontal flip for an image \cite{kanazawa2016warpnet}. While the idea of SSL is not new  \cite{bromley1993signature} the main focus has been on deep SSL models, which have been highly successful in domains such as computer vision \cite{chen2020simple,Jing2019SelfSupervisedVF} and natural language processing \cite{ misra2020self,BERT2019}.

\todo[inline]{todo: define exact forumation of the SSL model}
% \textbf{Standard embedding function.}


\subsection{Restricted Boltzmann Machine}
 Restricted Boltzmann Machine (RBM) is a type of stochastic artificial neural network that can learn a probability distribution over its set of inputs. It consists of two layers: a visible layer representing observable data, and a hidden layer representing latent variables. The key characteristic of an RBM is the restriction that there are no intra-layer connections; that is, the visible units are not connected to each other, and the hidden units are not connected to each other, only to units in the other layer.
 
\textbf{Setup:}
   Visible Units  $ {v} \in \mathbb{R}^n $.
   Hidden Units $ {h} \in \mathbb{R}^m $.
   Weights:$ W \in \mathbb{R}^{n \times m} $.
   Biases: Visible bias vector $ {a} \in \mathbb{R}^n $ and hidden bias vector $ {b} \in \mathbb{R}^m $.

\textbf{Energy Function:}
   The energy of a configuration $({v}, {h})$ is given by:
   \[
   E({v}, {h}) = -{v}^\top {a} - {h}^\top {b} - {v}^\top W {h}
   \]
   Here, $ {v}^\top {a} $ is the dot product of the visible units and their biases, $ {h}^\top {b} $ is the dot product of the hidden units and their biases, and $ {v}^\top W {h} $ represents the interaction between visible and hidden units.

\textbf{Probability Distributions:}
   The joint probability distribution over the visible and hidden units is:
     $
     P({v}, {h}) = \frac{1}{Z} \exp(-E({v}, {h}))
     $
     where $ Z $ is the partition function:
    $
     Z = \sum_{{v}} \sum_{{h}} \exp(-E({v}, {h})).
     $
The marginal probability of a visible vector $ {v} $ is:
     \begin{align*}
          P({v}) = \frac{1}{Z} \sum_{{h}} \exp(-E({v}, {h})).
     \end{align*}
    

\textbf{Optimization Problem}
The goal of training an RBM is to maximize the likelihood of the training data.
   The log-likelihood for a single data point $ {v} $ is:
   \[
   \mathcal{L}({v}) = \log P({v}) = \log \left( \sum_{{h}} \exp(-E({v}, {h})) \right) - \log Z
   \]
   Summing over the entire dataset $ \mathcal{D} = \{{v}^{(1)}, {v}^{(2)}, \ldots, {v}^{(N)}\} $, the log-likelihood is:
   \[
   \mathcal{L}(\mathcal{D}) = \sum_{{v} \in \mathcal{D}} \mathcal{L}({v})
   \]




% \subsection{Optimization}
% Before going into the numerical simulations we outline the details for the optimization for the above defined optimization problems.

% \textbf{Parameters.} The parameters of the model can be split into two main aspects. Firstly the parameters of the embedding function (e.g. the weights of the neural networks) and secondly, unique to the cluster specific representation learning setup we are interested in the optimization of $S$. For this part we again follow \cite{esser2023improved} and perform an itererative optimization of the form
% % \clearpage
% \begin{enumerate}
%     \item \textbf{Initialize} weights $\{\Phi_j, \Psi_j\}^k_{j},\Theta,\Omega$ and cluster assignments according to $k$-means ++ \cite{David2007kmeans}\footnote{The $k$-means ++ initialization scheme is not crucial however has been show to provide a better starting point then random initialization.}.
%     \item \textbf{Update the weights} for the (shared) encoder and (shared) decoder using a GD step.
%     \item \textbf{Update the class assignment} $S$ using a Lloyd’s step\footnote{Here the Lyod's step solves the linear problem on $S$ assuming all other parameters are fixed.} on a strict class-assignment.
% \end{enumerate}
% We iteratively repeat step 2 and 3 until convergence.

% \textbf{Hyper-parameter search.}

% \subsection{Inference}
% In a lot of applications of representation learning we are mainly interested in finding improved representations for a given dataset. However in some case we are also interested in finding embeddings of new data points, that where not considered in the training process (e.g. in denoising of data).
% %
% In contrast to AE, where one simply passes any new data through the trained network, TAE additionally decides on the latent variable $S$.
% Note then that essentially in our model the actual parameters are $\{\Phi_j, \Psi_j\}^k_{j},\Theta,\Omega$ whereas $S$ is simply an encoding of our confidence of what the latent variable or label is for each $X_i$. Thus to run the TAE on a new datapoint, we have to first estimate this latent variable.
% %
% Following this idea, let $S \in \mathbb{R}^k$, with its $j$'th coordinate being $S_j$.
% % \footnote{Note then that this is a linear problem in the variables $S_j$ and thus its solution is at some vertex of the bounding polytope, i.e. there is some $\hat{j}$ such that $\hat{S}_{\hat{j}} = 1$. Thus the label assigned to $\widetildeX_i$ is this $j$. } 
% Then given a new datapoint $X_i^*$ and given the trained parameters $\{\Phi_j, \Psi_j\}^k_{j},\Theta,\Omega$, we first find $\hat{S}$ such that 
% \begin{align*}
%     \hat{S} =& \argmin_{1_k^TS = 1; S_j \geq 0}  \sum^k_{j = 1} S_j g_{\Psi_j}\left(g_\Omega(X_i)\right).
% \end{align*}
% This general approach can be applied to all considered optimization problems to obtain the embedding for a new datapoint.



==> sections/results.tex <==
\section{Numerical Evaluation}
Having outlined the models we not numerically evaluate the performance on several tasks such as \emph{de-noising and clustering} as well as a qualitative analysis of the latent space learned by VAEs.
We show that partial tensorization reduces the model complexity compared to full tensorization without compromizing on performance.
\footnote{The code to reproduce the numerical simulations, including hyper parameter search, is provided in the supplemental material.}
\todo[inline]{for fig.\ref{fig:ae_clustering}:

1. add a plot next to it with number of parameters for different models (for one dataset should be enough)

2. Increase size of labels}
\todo[inline]{for fig.\ref{fig:ae_denoising}:

1. Increase size of labels}
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/AE/ae_clust_main_draft.pdf}
    \caption{ARI (higher is better) of different models}
    \label{fig:ae_clustering}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/AE/ae_denoise_main_draft.pdf}
    \caption{MSE (lower is better) De-noising of different models}
    \label{fig:ae_denoising}
\end{figure}

\subsection{De-Noising}

\subsection{Clustering}

\subsection{Latent space of VAE}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.24\linewidth]{figures/VAE/vae_lr0.001_ep200_reg0.5_mseFalse_loutFalse_clustidNone.pdf}
%     \includegraphics[width=0.24\linewidth]{figures/VAE/tvae_lr0.001_ep500_reg0.1_mseFalse_loutFalse_clustid0.pdf}
%     \includegraphics[width=0.24\linewidth]{figures/VAE/tvae_lr0.001_ep500_reg0.1_mseFalse_loutFalse_clustid1.pdf}
%     \includegraphics[width=0.24\linewidth]{figures/VAE/tvae_lr0.001_ep500_reg0.1_mseFalse_loutFalse_clustid2.pdf}
%     \caption{Sigmoid output, BCE loss, MNIST, FCN}
%     \label{fig:vae_latent_space}
% \end{figure*}


